On the Trajectory Regularity of ODE-based Diffusion Sampling

Diffusion-based generative models use stochastic differential equations (SDEs) and their equivalent ordinary differential equations (ODEs) to establish a smooth connection between a complex data distribution and a tractable prior distribution. In this paper, we identify several intriguing trajectory properties in the ODE-based sampling process of diffusion models. We characterize an implicit denoising trajectory and discuss its vital role in forming the coupled sampling trajectory with a strong shape regularity, regardless of the generated content. We also describe a dynamic programming-based scheme to make the time schedule in sampling better fit the underlying trajectory structure. This simple strategy requires minimal modification to any given ODE-based numerical solvers and incurs negligible computational cost, while delivering superior performance in image generation, especially in $5\sim 10$ function evaluations.

==> secs/magnitude.tex <==
\section{Visualization of High Dimensional Trajectory}
\label{sec:visual}
In this section, we present several tools to inspect the trajectory of probability flow ODE in high-dimensional space. We mostly take unconditional generation on CIFAR-10 as an example to demonstrate our observations. The conclusions also hold on other datasets (such as LSUN, ImageNet) and other model settings (such as conditional generation, various network architectures). More results and implementation details are provided in Appendix~\ref{app:exp}. 
% (such as CIFAR-10 \cite{krizhevsky2009learning}, LSUN \cite{yu2015lsun}, ImageNet \cite{russakovsky2015ImageNet})

%We adopt $d(\cdot, \cdot)$ to denote the $\ell_2$ distance. Take the sampling trajectory as an example, the distance between a given sample $\hatx_{t_n}$ and the final sample $\hatx_{t_0}$ is denoted as $d(\hatx_{t_n}, \hatx_{t_0})$. The \textit{trajectory deviation} is calculated as the distance between each intermediate sample $\hatx_{t_n}$ and the straight line passing through two endpoints $\left[\hatx_{t_0}\hatx_{t_N}\right]$, and denoted as $d(\hatx_{t_n}, \left[\hatx_{t_0}\hatx_{t_N}\right])$. 
The expectation quantities (\textit{e.g.}, distance, magnitude) in every time steps are estimated by averaging 50k generated samples. 
%and plot the average distance at each time step. 

\subsection{Forward Diffusion Process}
\label{subsec:norm}
As discussed in Section~\ref{sec:background}, the forward process is generally interpreted as a progressive smoothing from data to noise with a series of Gaussian perturbation kernels. We further paraphrase it as the expansion of magnitude and manifold, which means that %for each diffusion step, 
samples escape from the original \textit{small-magnitude low-rank} manifold and settle into a \textit{large-magnitude high-rank} manifold. 
%The following proposition gives us a glimpse of the geometric structure in high dimensions
\begin{proposition}
	\label{prop:norm}
	Given a high-dimensional vector $\bfx \in \bbR^d$ and an isotropic Gaussian noise $\bfz \sim \calN(\mathbf{0} ; {\sigma^2\bfI_d})$, $\sigma>0$, we have $\bbE \left\lVert \bfz \right\rVert^2=\sigma^2 d$, and with high probability, $\bfz$ stays within a ``thin shell'': $\lVert \bfz \rVert = \sigma \sqrt{d} \pm O(1)$. Additionally, $\bbE \left\lVert \bfx + \bfz \right\rVert ^2 =\lVert \bfx \rVert^2 +  \sigma^2d$, 
	$\lim_{d\rightarrow \infty}\bbP \left( \lVert \bfx + \bfz  \rVert > \lVert \bfx \rVert \right)=1$. 
\end{proposition}
The proofs are provided in Appendix~\ref{app:norm}. Proposition~\ref{prop:norm} implies that in the forward process, the squared magnitude of the noisy sample $\bfx +\bfz$ is expected to be larger than that of the original sample $\bfx$, and their magnitude gap becomes especially huge for the high-dimensional case $d\gg 1$ and severe noise case $\sigma \gg 0$. 
We can further conclude that as $d\rightarrow \infty$, the sample magnitude will expand with probability one and the isotropic Gaussian noise will distribute as a uniform distribution on the sphere \cite{vershynin2018high}.
%, due to the \textit{concentration of measure}  
In practical generative modeling, $d$ is sufficiently large to make this claim approximately correct. The low-rank data manifold is thus lifted to about $d-1$ rank sphere of radius $\sigma\sqrt{d}$, with a thin shell of width $O(1)$. 
%\textit{i.e.}, $\bfz\sim\text{Unif}(\sigma \sqrt{d} \, \calS^{d-1})$, 
%it follows the \textit{quadratic relation} w.r.t the noise scale. 
In Figure~\ref{fig:magnitude}, we track the magnitude of original data in the forward process and the magnitude of synthetic samples in the backward process. A clear trend is that the sample magnitude expands in the forward diffusion process and shrinks in the backward generative process, and they are well-matched thanks to the marginal preserving property.
%\cite{song2021sde}. 
%(the pixel values are re-scaled to $[-1,1]$)


%Due to the marginal preserving property of PF-ODE \cite{song2021sde}, the backward process behaves in a magnitude shrinking fashion and the analysis is similar. 

%Furthermore, the isotropic Gaussian noise is distributed around the sphere of radius (about $4433 \pm 57$), which is significantly larger than the original data in magnitude (about $27 \pm 7$).
